Wigner-Smith Time Delay Matrix for Electromagnetics: Computational Aspects for Radiation and Scattering Analysis

The WS time delay matrix relates a lossless and reciprocal system's scattering matrix to its frequency derivative, and enables the synthesis of modes that experience well-defined group delays when interacting with the system. The elements of the WS time delay matrix for surface scatterers and antennas comprise renormalized energy-like volume integrals involving electric and magnetic fields that arise when exciting the system via its ports. Here, direct and indirect methods for computing the WS time delay matrix are presented. The direct method evaluates the energy-like volume integrals using surface integral operators that act on the incident electric fields and current densities for all excitations characterizing the scattering matrix. The indirect method accomplishes the same task by computing scattering parameters and their frequency derivatives. Both methods are computationally efficient and readily integrated into existing surface integral equation codes. The proposed techniques facilitate the evaluation of frequency derivatives of antenna impedances, antenna patterns, and scatterer radar cross sections in terms of renormalized field energies derived from a single frequency characterization of the system.

==> graphics/fig_Loop.tex <==
\begin{tikzpicture}[valign=t, thick,scale=0.7, every node/.style={scale=0.7}]
\centering
\draw[fill=black!40] (0,0) rectangle (6,3);
\draw[fill=white] (0.1,0.1) rectangle (5.9,2.9);
\draw[red, line width =2mm] (0,1.5) -- (0.1,1.5);
\node at (0.4,1.5) [right] {antenna port};
\draw [->] (0.4, 1.5) -- (0.1,1.5);
\draw [<->] (0,-0.1) -- (6,-0.1);
\node at (3,-0.1) [below] { 300~mm};
\draw [<->] (-0.1,0) -- (-0.1,3);
\node at (-0.0,1.5) [left] { 150~mm};

\draw [<->] (0.1,0.2) -- (5.9,0.2);
\node at (3,0.2) [above] { 290~mm};
\end{tikzpicture}


==> graphics/flow_chart.tex <==
%\documentclass{standalone}
%\usepackage{tikz} 
%\usepackage{graphicx}
%\usepackage{pgfplots}

%\begin{document}

\begin{tikzpicture}[thick,scale=0.7, every node/.style={scale=1}]
\setlength{\tabcolsep}{4pt}

\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle,draw,inner sep=0.5pt] (char) {#1};}}
            
            
            
\begin{scope}[shift={(0.5,0)}]            
\draw [rounded corners=5pt, fill=black!20](-2.4,-1) rectangle (2.4,1);
\node at (0.0,0) { \begin{tabular}{l} \circled{1} PEC \\  Radiator/Scatterer
\end{tabular}};
\end{scope}

\node at (3.75,0) {\tikzfancyarrow[0.75cm]{}};

%\node[draw,circle] at (0,0) {1};

\begin{scope}[shift={(7.0,0)}]
\draw [rounded corners=5pt, fill=black!20](-2.4,-1) rectangle (2.4,1);
\node at (0.0,0) { \begin{tabular}{l} \circled{2} SIE analysis \\ for all excitations\\
 $\vect{\cal E}_p^{\text{inc}}(r) \rightarrow \vect{\cal J}_p(r)$
\end{tabular}};
\end{scope}


\node at (0.3,-2.5) {\tikzfancyarrow[0.75cm]{}};

\begin{scope}[shift={(3.5,-2.5)}]
\draw [rounded corners=5pt, fill=black!20](-2.4,-1) rectangle (2.4,1);
\node at (0.0,0) { \begin{tabular}{l} \circled{3} SI \\  computation \\ of $\matr{Q}$ and $\matr{S}$
\end{tabular}};
\end{scope}


\node at (-1.8,-5) {\tikzfancyarrow[0.75cm]{}};

\begin{scope}[shift={(0.9,-5)}]
\draw [rounded corners=5pt, fill=black!20](-2,-1) rectangle (2,1);
\node at (0.0,0) { \begin{tabular}{c} \circled{4} $\dfrac{d \matr{S}}{d \omega} = - j \matr{S} \matr{Q}$
\end{tabular}};
\end{scope}


\node at (3.8,-5) {\tikzfancyarrow[0.75cm]{}};


\begin{scope}[shift={(6.6,-5)}]
\draw [rounded corners=5pt, fill=black!20](-2,-1) rectangle (2,1);
\node at (0.0,0) {\circled{5}  $\dfrac{\partial}{d \omega}\begin{bmatrix} \matr{Z} \\ \text{far-field} \\ \text{RCS} \end{bmatrix}$ 
};
\end{scope}


\end{tikzpicture}

%\end{document}

==> graphics/scattering_system.tex <==
\begin{figure}
\centering
\begin{circuitikz}
\draw (0,0) circle (2.5);
\draw[dashed] (0,0) circle (1.4);

\draw[fill=black] (0,0) circle (0.02);

\draw[fill=black!40] (-0.6,0.02) rectangle (-0.4,1.2);
\draw (-0.6,-0.02) rectangle (-0.4,0.02);
\draw[fill=black!40] (-0.6,-0.02) rectangle (-0.4,-1.2);
\draw (-0.6,-0.02) rectangle (-0.4,0.02);
\draw[fill=black!40] (0.6,0.02) rectangle (0.4,1.2);




\draw[fill=black!40] (0.6,0.02) rectangle (0.4,1.2);
\draw[fill=black!40] (0.6,-0.02) rectangle (0.4,-1.2);
\draw (0.6,-0.02) rectangle (0.4,0.02);

\begin{scope}[scale =0.2, shift={(-0.2,3)}]
\draw [black, fill = black!60] plot [smooth cycle] coordinates {(1.9,0)  (1.6, 0.9) (1.0, 1.2) (0.5, 1.25) (0,1) (-0.5,0.8) (-0.7, 0.65) (-1,0) (-0.8, -0.6) (-0.5,-0.8) (0,-0.9) (0.5, -1)  (1.5, -0.8)};
\end{scope}
\draw[fill = black!60] (-0.75,0.8) circle (0.1);
\draw[fill = black!60] (-0.85,0.5) ellipse (0.15 and 0.1);

\begin{scope}[scale =0.22, shift={(-5.2,-0.6)}]
\draw [black, fill = black!60] plot [smooth cycle] coordinates {(1.9,0)  (1.6, 0.9) (1.0, 1.2) (0.5, 1.25) (0,1) (-0.5,0.8) (-0.7, 0.65) (-1,0) (-0.8, -0.6) (-0.5,-0.8) (0,-0.9) (0.5, -1)  (1.5, -0.8)};
\end{scope}



%\node at (180:3.25) [left] {$d\Omega$};
\foreach \th in {40, 80, 120, ..., 360}
{
\draw [->] (\th:2.7) -- (\th:2.5);
\draw [->] (\th-5:2.5) -- (\th-5:2.7);
}
\node at (-1.8,1.5) [right] {\small $d\Omega_\circ$};
\draw[->] (139:2.3) -- (142:2.45);
%\draw[->] (140:2) -- (-1,0.78);
%\draw[->] (140:2) -- (-1,-0.7);


\draw[->] (3,1) -- (0.605,0.0);
\draw[dashed, blue] (0.37, -0.06) rectangle (0.63, 0.06);

\begin{scope}[scale = 0.5, shift={(7, 2)}, every node/.style={scale=0.4}]

\draw[dashed] (-1.1, -2.5) rectangle (6.5, 3.5); 
\draw[fill=black!40] (-0.35,0) rectangle (0.15,-2);
\draw[fill=black!40] (-0.35,1.25) rectangle (0.15,3.25);

\draw[pattern=dots] (-0.35,0) rectangle (0.15, 1.25);
\node at (-0.7,1.5) {\Large $d\Omega_p$};
\draw[->] (-0.6,1.25) -- (0,0.5);

\begin{scope}[shift={(1,0)}]

\draw (-1,0) -- (0,0)  to[TL, o-o] (3,0);
\draw (-1,1.25) -- (0,1.25)  to[TL, o-o] (3,1.25);
\draw (3,0) to (4.5,0) to[vsourcesin, o-o] (4.5,1.25)   to[R,o-o] (3,1.25);
\draw[<-|] (0.25,1.75) -- (2.5,1.75);
\node at (2.4, 2.0) [above] {\Large $w=0$};
\node at (0.75, 2.0) [above] {\Large $w=d$};
\node at (3.5,1.75) {\Large $Z_o$};
\node at (1.5,0.6) {\Large $Z_o$};
\node at (4.75,0.625) [right] {\Large $V_{p}$};
\draw[dashed] (3,-1.5) -- (3,2.5);
\node at (3,-1.5) [below] {\Large  \begin{tabular} \,Reference \\Plane\end{tabular}};
\draw [->] (3.5,-0.5) -- (2.5,-0.5);
\draw[->] (2.5,-1) -- (3.5,-1); 
\node at (3.5,-1) [right] {\Large $b_p$};
\node at (2.5,-0.5) [left] {\Large $a_p$};
%\draw[<->] (0,0.0) -- (0,1.2);
\end{scope}
\end{scope}

\node at (50:2.0) [above] {\small $R$};
\node at (0,-2) {\small $\Omega$};
\draw[->] (0,0) -- (45:2.5);


\draw[->] (0,0) -- (340:1.4);
\node at (340:1.2) [above] {\small $a$};
%\node at (-2.5,0) {\begin{tabular}{c} physical\\ ports \end{tabular}};
%\draw[->] (-2.3,0.4) -- (-1,0.6);
%\draw[->] (-2.3,-0.4) -- (-1,-0.8);




\end{circuitikz}
\caption{Radiating system excited by lumped voltage source and free-space ports.}
\label{fig:mixed_scatterer}
\end{figure}
